Faithful Persona-based Conversational Dataset Generation with Large Language Models

High-quality conversational datasets are essential for developing AI models that can communicate with users. One way to foster deeper interactions between a chatbot and its user is through personas, aspects of the user's character that provide insights into their personality, motivations, and behaviors. Training Natural Language Processing (NLP) models on a diverse and comprehensive persona-based dataset can lead to conversational models that create a deeper connection with the user, and maintain their engagement. In this paper, we leverage the power of Large Language Models (LLMs) to create a large, high-quality conversational dataset from a seed dataset. We propose a Generator-Critic architecture framework to expand the initial dataset, while improving the quality of its conversations. The Generator is an LLM prompted to output conversations. The Critic consists of a mixture of expert LLMs that control the quality of the generated conversations. These experts select the best generated conversations, which we then use to improve the Generator. We release Synthetic-Persona-Chat, consisting of 20k conversations seeded from Persona-Chat. We evaluate the quality of Synthetic-Persona-Chat and our generation framework on different dimensions through extensive experiments, and observe that the losing rate of Synthetic-Persona-Chat against Persona-Chat during Turing test decreases from 17.2% to 8.8% over three iterations.

==> notes.tex <==
experiment 1: The persona expansion model is able to augment  seed persona set while keeping the diversity and specificty of the 
increases the number of personsas by 100 percent while maintaining the original persona categories and adding 265 new persona categories. The new geenrated personas are longer by average 50percent per persona which can be interpreted as including more details in the new personas. 
be more quantitate in the observations. and advertise using those numbers.
Experiment 2: coherent --> 
tha improvement in which type of method:
1. next utterance --> sanitity check for coherence
2. use models to find the complexity of the conversations. word overlap vs concept overlap
compare them row based in table 2. relative improvements between models. 
PC people just copied the utterance --> PC+ requires reasonign and transformers compared to IR baseline

Table 3:
why those numbers are so high --> maybe task is easy
increase the number of distractors --> use statistic sets --> make task really hard
using the other speaker in PC+ -- > This is really weak 
find the humanness reference and change it to Turning test

Use the third column which shows they are equal 
Diversity details should be in the appendix (chart of each charachteristics) and just keep the statement
strong profanity gets better, but potential profanity mehhh based on their confidence value


Rewrite the experiment section and use quantitative section... --> then pic 5 favorite advantages of pc+ and add them to intro. 
Use inclusive in advertising
